Full asymptotic expansion for Polya structures

In order to obtain the full asymptotic expansion for Polya trees, i.e. rooted unlabelled and non-plane trees, Flajolet and Sedgewick observed that their specification could be seen as a slight disturbance of the functional equation satisfied by the Cayley tree function. Such an approach highlights the complicated formal expressions with some combinatorial explanation. They initiated this process in their book but they spared the technical part by only exhibiting the first- order approximation. In this paper we exhibit the university of the method and obtain the full asymptotic expansions for several varieties of trees. We then focus on three different varieties of rooted, unlabelled and non-plane trees, Polya trees, rooted identity trees and hierarchies, in order to calculate explicitly their full singular expansions and asymptotic expansions.

==> header.tex <==
\pagestart{1}

\pageend{12}
\authorhead{Antoine Genitrini}
\titlehead{Full asymptotic expansion for P\'olya structures}
\titlelong{Full asymptotic expansion for P\'olya structures}
\keywords{Unlabelled non-plane trees; Full Puiseux expansion; Full asymptotic expansion; Analytic Combinatorics.}


